Building Embedded Systems Like It's 1996

Embedded devices are ubiquitous. However, preliminary evidence shows that attack mitigations protecting our desktops/servers/phones are missing in embedded devices, posing a significant threat to embedded security. To this end, this paper presents an in-depth study on the adoption of common attack mitigations on embedded devices. Precisely, it measures the presence of standard mitigations against memory corruptions in over 10k Linux-based firmware of deployed embedded devices. The study reveals that embedded devices largely omit both user-space and kernel-level attack mitigations. The adoption rates on embedded devices are multiple times lower than their desktop counterparts. An equally important observation is that the situation is not improving over time. Without changing the current practices, the attack mitigations will remain missing, which may become a bigger threat in the upcoming IoT era. Throughout follow-up analyses, we further inferred a set of factors possibly contributing to the absence of attack mitigations. The exemplary ones include massive reuse of non-protected software, lateness in upgrading outdated kernels, and restrictions imposed by automated building tools. We envision these will turn into insights towards improving the adoption of attack mitigations on embedded devices in the future.

==> defs.tex <==
\usepackage{xparse}
\newcommand{\bnm}{\begin{newmath}}
\newcommand{\enm}{\end{newmath}}

\newcommand{\bea}{\begin{eqnarray*}}%
\newcommand{\eea}{\end{eqnarray*}}%

\newcommand{\bne}{\begin{newequation}}
\newcommand{\ene}{\end{newequation}}

\newcommand{\bal}{\begin{newalign}}
\newcommand{\eal}{\end{newalign}}

\newenvironment{newalign}{\begin{align}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{align}}

\newenvironment{newmath}{\begin{displaymath}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{displaymath}}

\newenvironment{neweqnarrays}{\begin{eqnarray*}%
\setlength{\abovedisplayskip}{-4pt}%
\setlength{\belowdisplayskip}{-4pt}%
\setlength{\abovedisplayshortskip}{-4pt}%
\setlength{\belowdisplayshortskip}{-4pt}%
\setlength{\jot}{-0.4in} }{\end{eqnarray*}}

\newenvironment{newequation}{\begin{equation}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{equation}}


\newcounter{ctr}
\newcounter{savectr}
\newcounter{ectr}

\newenvironment{newitemize}{%
\begin{list}{\mbox{}\hspace{5pt}$\bullet$\hfill}{\labelwidth=15pt%
\labelsep=4pt \leftmargin=12pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{3pt} }}{\end{list}}


\newenvironment{newenum}{%
\begin{list}{{\rm (\arabic{ctr})}\hfill}{\usecounter{ctr} \labelwidth=17pt%
\labelsep=5pt \leftmargin=22pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{2pt} }}{\end{list}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Figure and table macros
%

\newcounter{mytable}
\def\mytable{\begin{centering}\refstepcounter{mytable}}
\def\endmytable{\end{centering}}

\def\mytablecaption#1{\vspace{2mm}
  \centerline{Table \arabic{mytable}.~{#1}}
  \vspace{6mm}
  \addcontentsline{lot}{table}{\protect\numberline{\arabic{mytable}}~{#1}}
}


\newcounter{myfig}
\def\myfig{\begin{centering}\refstepcounter{myfig}}
\def\endmyfig{\end{centering}}

\def\myfigcaption#1{
             \vspace{2mm}
             \centerline{\textsf{Figure \arabic{myfig}.~{#1}}}
             \vspace{6mm}
             \addcontentsline{lof}{figure}{\protect\numberline{\arabic{myfig}}~{#1}}}


\newlength{\saveparindent}
\setlength{\saveparindent}{\parindent}
\newlength{\saveparskip}
\setlength{\saveparskip}{\parskip}

\newcommand{\decOracle}{\textbf{Dec}}

\newcommand{\negsmidge}{{\hspace{-0.1ex}}}
\newcommand{\cdotsm}{\negsmidge\negsmidge\negsmidge\cdot\negsmidge\negsmidge\negsmidge}

\def\suchthatt{\: :\:}
\newcommand{\E}{{\rm I\kern-.3em E}}
\newcommand{\Prob}[1]{{\Pr\left[\,{#1}\,\right]}}
\newcommand{\Probb}[2]{{\Pr}_{#1}\left[\,{#2}\,\right]}
\newcommand{\CondProb}[2]{{\Pr}\left[\: #1\:\left|\right.\:#2\:\right]}
\newcommand{\CondProbb}[2]{\Pr[#1|#2]}
\newcommand{\ProbExp}[2]{{\Pr}\left[\: #1\:\suchthatt\:#2\:\right]}
\newcommand{\Ex}[1]{{\textnormal{E}\left[\,{#1}\,\right]}}
\newcommand{\Exx}{{\textnormal{E}}}
\newcommand{\given}{\ensuremath{\,\big|\,}}


\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}
\def\negl{\mathsf{negl}}


\newcommand{\secref}[1]{\mbox{Section~\ref{#1}}}
\newcommand{\appref}[1]{\mbox{Appendix~\ref{#1}}}
\newcommand{\thref}[1]{\mbox{Theorem~\ref{#1}}}
\newcommand{\defref}[1]{\mbox{Definition~\ref{#1}}}
\newcommand{\corref}[1]{\mbox{Corollary~\ref{#1}}}
\newcommand{\lemref}[1]{\mbox{Lemma~\ref{#1}}}
\newcommand{\clref}[1]{\mbox{Claim~\ref{#1}}}
\newcommand{\propref}[1]{\mbox{Proposition~\ref{#1}}}
\newcommand{\factref}[1]{\mbox{Fact~\ref{#1}}}
\newcommand{\remref}[1]{\mbox{Remark~\ref{#1}}}
\newcommand{\figref}[1]{\mbox{Figure~\ref{#1}}}
\renewcommand{\algref}[1]{\mbox{Algorithm~\ref{#1}}}
% \newcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
% Have to use \renewcommand because exists already in amsmath
\renewcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
\newcommand{\consref}[1]{\mbox{Construction~\ref{#1}}}
\newcommand{\tabref}[1]{\mbox{Table~\ref{#1}}}

\newcommand{\get}{{\:{\leftarrow}\:}}
\newcommand{\gett}[1]{\:{\leftarrow}_{#1}\:}
\newcommand{\getsr}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle\$$}}}\:}}
\newcommand{\getm}{{\:\leftarrow_{\mdist}\:}}
\newcommand{\getd}{{\:\leftarrow_{\ddist}\:}}
%\newcommand{\getm}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle \mdist$}}}\:}}
\newcommand{\getk}{{\:\leftarrow_{\kdist}\:}}
%\newcommand{\getk}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle \kdist$}}}\:}}
\newcommand{\getp}{{\:\leftarrow_{p}\:}}



\newcommand{\gamesfontsize}{\small}
\newcommand{\fpage}[2]{\framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}}
\newcommand{\mpage}[2]{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}

\newcommand{\hpages}[3]{\begin{tabular}{cc}\begin{minipage}[t]{#1\textwidth} #2 \end{minipage} & \begin{minipage}[t]{#1\textwidth} #3 \end{minipage}\end{tabular}}

\newcommand{\hpagess}[4]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #3 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #4 \end{minipage}
        \end{tabular}
    }

\newcommand{\hpagesss}[6]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #4 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #5 \end{minipage}
        &
        \begin{minipage}[t]{#3\textwidth}\gamesfontsize #6 \end{minipage}
        \end{tabular}
    }

\newcommand{\hpagessss}[8]{
        \begin{tabular}{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #5 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #6 \end{minipage}
        &
        \begin{minipage}[t]{#3\textwidth}\gamesfontsize #7 \end{minipage}
        &
        \begin{minipage}[t]{#4\textwidth}\gamesfontsize #8 \end{minipage}
        \end{tabular}
    }


\newcommand{\hfpages}[3]{\hfpagess{#1}{#1}{#2}{#3}}
\newcommand{\hfpagess}[4]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #3 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
        \end{tabular}
    }
\newcommand{\hfpagesss}[6]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #5 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.1}\gamesfontsize #6 \end{minipage}}
        \end{tabular}
    }
\newcommand{\hfpagessss}[8]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #5 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #6 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.1}\gamesfontsize #7 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#4\textwidth}\setstretch{1.1}\gamesfontsize #8 \end{minipage}}
        \end{tabular}
    }

\newcommand{\vecw}{\mathbf{w}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\load}{L}
\newcommand{\coll}{\mathsf{Coll}}
\newcommand{\nocoll}{\overline{\mathsf{Coll}}}


\newcommand{\Img}{\textsf{Img}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Fonts and symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\funcfont{\textsf}
\newcommand\variablefont{\texttt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NEW COMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def \Perm {\funcfont{Perm}}
\def \calC {{\mathcal{C}}}
\def \calU {{\mathcal{U}}}
\renewcommand{\u}{\ensuremath{u}}
\newcommand{\unew}{\ensuremath{\tilde{u}}}

\newcommand{\calN}{\mathcal{N}}
\def \sspace {{\mathcal{S}}}
\def \strings {{\mathcal{S}}}
\def \slen {{s}}
\def \kspace {{\mathcal{K}}}
\def \kspacesize {{m}}
\def \mspacesize {{n}}
\def \kdict {D}
\def \dictsize {d}
\newcommand{\kdist}{p_k}
\newcommand{\mdist}{\ensuremath{{W}}}
\newcommand{\alldist}{\rho}
\newcommand{\pwdist}{\transgen}
\newcommand{\ddist}{\rho_{dec}}
\newcommand{\PWset}{{\mathcal{P}}}  % TODO: fix, same as \pwdist
\newcommand{\PWsetvec}{\vec{\mathcal{P}}}
\newcommand{\PWvec}{\vec{P}}
\newcommand{\domvec}{\vec{D}}
\newcommand{\humanornot}{\vec{h}}
\newcommand{\dom}{\textsf{dom}}
%\def \kdist {{\kappa}}
%\def \mdist {{\mu}}
%\def \ddist {{\delta}}
\def \pspace {{\mathcal{P}}}
\def \mpspace {{\mathcal{MP}}}
\def \cspace {{\mathcal{C}}}
\def \key {\kappa}
\def \msg {M}
\def \seed {S}
\def \ctxt {C}
\def \ctxtpart {C_2}
\newcommand{\genprime}{{\textsf{GenPrime}}}
\newcommand{\isprime}{{\textsf{IsPrime}}}
\newcommand{\LeastLesserPrime}{{\textsf{PrevPrime}}}
\newcommand{\pwset}{\mathcal{S}}
\newcommand{\DTE}{{\textsf{DTE}}}
\newcommand{\encode}{{\textsf{encode}}}
\newcommand{\decode}{{\textsf{decode}}}

\newcommand{\DTEsingle}{{\textsf{1PW-DTE}}}
\newcommand{\encodesingle}{{\textsf{1PW-encode}}}
\newcommand{\decodesingle}{{\textsf{1PW-decode}}}

\newcommand{\DTErss}{{\textsf{RSS-DTE}}}
\newcommand{\encoderss}{{\textsf{RSS-encode}}}
\newcommand{\decoderss}{{\textsf{RSS-decode}}}

\newcommand{\DTEindep}{{\textsf{MPW-DTE}}}
\newcommand{\encodeindep}{{\textsf{MPW-encode}}}
\newcommand{\decodeindep}{{\textsf{MPW-decode}}}


\newcommand{\DTEsub}{{\textsf{SG-DTE}}}
\newcommand{\encodesub}{{\textsf{SG-encode}}}
\newcommand{\decodesub}{{\textsf{SG-decode}}}
\newcommand{\decodekamf}{{\textsf{KAMF-decode}}}
\newcommand{\DTEis}{{\textsf{IS-DTE}}}
\newcommand{\encodeis}{{\textsf{is-encode}}}
\newcommand{\decodeis}{{\textsf{is-decode}}}
\newcommand{\DTErej}{{\textsf{REJ-DTE}}}
\newcommand{\encoderej}{{\textsf{rej-encode}}}
\newcommand{\decoderej}{{\textsf{rej-decode}}}
\newcommand{\DTErsarej}{{\textsf{RSA-REJ-DTE}}}
\newcommand{\encodeRSAREJ}{{\textsf{rsa-rej-encode}}}
\newcommand{\decodeRSAREJ}{{\textsf{rsa-rej-decode}}}
\newcommand{\DTErsainc}{{\textsf{RSA-INC-DTE}}}
\newcommand{\encodeRSAINC}{{\textsf{rsa-inc-encode}}}
\newcommand{\decodeRSAINC}{{\textsf{rsa-inc-decode}}}
\newcommand{\DTEunf}{{\textsf{UNF-DTE}}}
\newcommand{\DTEnunf}{{\textsf{NUNF-DTE}}}


%\newcommand{\encodeis}{{\textsf{encode}_{\textrm{is}}}}
%\newcommand{\decodeis}{{\textsf{decode}_{\textrm{is}}}}
\newcommand{\rep}{\textsf{rep}}
\newcommand{\isErr}{\epsilon_{\textnormal{is}}}
\newcommand{\incErr}{\epsilon_{\textnormal{inc}}}
\def \enc {{\textsf{E}}}
\def \dec {{\textsf{D}}}
\def \SEscheme {{\textsf{SE}}}
\def \HEscheme {{\textsf{HE}}}
\def \CTR {{\textsf{CTR}}}
\def \encHE {{\textsf{HEnc}}}
\def \HIDE {{\textsf{HiaL}}}
\def \encHIDE {{\textsf{HEnc}}}
\def \decHIDE {{\textsf{HDec}}}
\def \decHE {{\textsf{HDec}}}
\def \encHEt {{\textsf{HEnc2}}}
\def \decHEt {{\textsf{HDec2}}}

\newcommand{\myind}{\hspace*{1em}}
\newcommand{\thh}{^{\textit{th}}} % th
\newcommand{\concat}{\,\|\,}
\newcommand{\dotdot}{..}
\newcommand{\emptystr}{\varepsilon}

\newcommand{\round}{\textsf{round}}

\newcommand{\alphabar}{\overline{\alpha}}
\newcommand{\numbinsbar}{\overline{b}}
\newcommand{\numballs}{a}
\newcommand{\numbins}{b}

%\def \encHE {{\sf{enc}^{HE}}}
%\def \decHE {{\sf{dec}^{HE}}}
%\def \encHEt {{\sf{enc}^{HE2}}}
%\def \decHEt {{\sf{dec}^{HE2}}}
\def \idealHE {{\mathcal{HE}}}
\def \IEnc {{\mathbf{\rho}}}
\def \IDec {{\mathbf{\rho^{-1}}}}
\def \OEnc {{\mathbf{Enc}}}
\def \ODec {{\mathbf{Dec}}}
\newcommand{\SimuProc}{\mathbf{Sim}}
\newcommand{\ROProc}{\mathbf{RO}}
\newcommand{\PrimProc}{\mathbf{Prim}}
\def \stm {g}
\def \istm {\hat{g}}
\def \kts {{f}}
\def \lex {{\sf lex}}
\def \part {part}
\def \kd {{\sf{kd}}}
\def \msgdist {{d}}
\def \keydist {{r}}
\def \ind {{\sf{index}}}
\def \kprf {z}
\def \adv {{\mathcal A}}
\def \pwds {u}
\newcommand{\mpw}{mpw}
\newcommand{\pw}{w}
\newcommand{\pwvec}{\vec{\pw}}
\newcommand{\vecx}{\vec{x}}
\def \tokens {v}
\def \calP{{\mathcal{P}}}
\def \template{{\mathcal{T}}}
\def \vaultset{{\mathcal{V}}}
\def \ext {{\sf ext}}
\def \offset {\delta}
\def \maxweight {\epsilon}
\def \advo {{\mathcal{A}}^{*}}

\newcommand{\Chall}{\textsf{Ch}}
\newcommand{\Test}{\textnormal{\textsf{Test}}}
\newcommand{\RoR}{\textsf{RoR}}
\newcommand{\MI}{\textnormal{MI}}
\providecommand{\MR}{\textnormal{MR}}
\newcommand{\MRCCA}{\textnormal{MR-CCA}}
\newcommand{\SAMP}{\textnormal{SAMP}}
\newcommand{\DTEgame}{\textnormal{SAMP}}
\newcommand{\KR}{\textnormal{KR}}
\newcommand{\advA}{{\mathcal{A}}}
\newcommand{\advR}{{\mathcal{R}}}
\newcommand{\advB}{{\mathcal{B}}} % 
\newcommand{\advC}{{\mathcal{C}}} % C
\newcommand{\advD}{{\mathcal{D}}} % D
\newcommand{\advE}{{\mathcal{E}}}
\newcommand{\advF}{{\mathcal{F}}}
\newcommand{\advG}{{\mathcal{G}}}
\newcommand{\advI}{{\mathcal{I}}}
\newcommand{\nextval}{\;;\;}
\newcommand{\TabC}{\texttt{C}}
\newcommand{\TabR}{\texttt{R}}
\newcommand{\Hash}{H}
\newcommand{\Cipher}{\pi}
\newcommand{\CipherInv}{\pi^{-1}}
\newcommand{\simu}{{\mathcal S}}
\newcommand{\prim}{P}
\newcommand{\maxguess}{\gamma}


\newcommand{\bigO}{\mathcal{O}}
\newcommand{\calG}{{\mathcal{G}}}

\def\sqed{{\hspace{5pt}\rule[-1pt]{3pt}{9pt}}}
\def\qedsym{\hspace{2pt}\rule[-1pt]{3pt}{9pt}}

\newcommand{\Colon}{{\::\;}}
\newcommand{\good}{\textsf{Good}}

\newcommand\Tvsp{\rule{0pt}{2.6ex}}
\newcommand\Bvsp{\rule[-1.2ex]{0pt}{0pt}}
\newcommand{\TabPad}{\hspace*{5pt}}
\newcommand\TabSep{@{\hspace{5pt}}|@{\hspace{5pt}}}
\newcommand\TabSepLeft{|@{\hspace{5pt}}}
\newcommand\TabSepRight{@{\hspace{5pt}}|}


\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\comma}{\textnormal{,}}

\renewcommand{\paragraph}[1]{\vspace*{6pt}\noindent\textbf{#1}\;}

\newcommand{\weirvault}{\textsf{Pastebin}\xspace}
\newcommand{\ndssvault}{\textsf{DBCBW}\xspace}




\newcommand{\reminder}[1]{ [[[ \marginpar{\mbox{$<==$}} #1 ]]] }

%
% New theorem types: (Already in CCS template)
%
\newtheorem{observation}{Observation}
%\newtheorem{definition}{Definition}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{fact}{Fact}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{corollary}{Corollary}[section]
% \newtheorem{proposition}{Proposition}
% \newtheorem{example}{Example}

%
% Definitions:
%
\def \blackslug{\hbox{\hskip 1pt \vrule width 4pt height 8pt
    depth 1.5pt \hskip 1pt}}
\def \qed{\quad\blackslug\lower 8.5pt\null\par}
% In-line QED, for ending a proof with a $$ formula
% In-line QED, for ending a proof with a $$ formula
\def \inQED{\quad\quad\blackslug}
\def \Qed{\QED}
\def \QUAD{$\Box$}
\def \Proof{\par\noindent{\bf Proof:~}}
\def \proof{\Proof}
\def \poly {\mbox{$\mathsf{poly}$}}
\def \binary {\mbox{$\mathsf{binary}$}}
\def \ones {\mbox{$\mathsf{ones}$}}
\def \rank {\mbox{$\mathsf{rank}$}}
\def \bits {\mbox{$\mathsf{bits}$}}
\def \factorial {\mbox{$\mathsf{factorial}$}}
\def \fr {\mbox{$\mathsf{fr}$}}
\def \pr {\mbox{$\mathsf{pr}$}}
\def \zon {\{0,1\}^n}
\def \zo  {\{0,1\}}
\def \zok {\{0,1\}^k}
\def \mo {s}


\def\utilcnt{\ensuremath{\mu_{\mathrm{cnt}}}}
\def\utiltime{\ensuremath{\mu_{\mathrm{time}}}}
\def\ex{\ensuremath{{\mathrm{ex}}}}
\def\rlx{\ensuremath{{\mathrm{rlx}}}}
\def\tp{\textsf{TP}}
\def\cp{\textnormal{\textsf{CP}}\xspace}
\def\edistcutoff{\edist}
\def\entcutoff{\ensuremath{m}}
\def\relentcutoff{{\sigma}}
\def\mutt{\mu_{\mathrm{tt}}}

\newcommand{\Hdot}{H(\mbox{ } \cdot \mbox{ }  , \mbox{ } \del)}


\newcounter{mynote}[section]
\newcommand{\notecolor}{blue}
\newcommand{\thenote}{\thesection.\arabic{mynote}}
\newcommand{\tnote}[1]{\refstepcounter{mynote}{\bf \textcolor{\notecolor}{$\ll$TomR~\thenote: {\sf #1}$\gg$}}}

\newcommand{\fixme}[1]{{\textcolor{red}{[FIXME: #1]}}}
\newcommand{\todo}[1]{{\textcolor{red}{[TODO: #1]}}}


\newcommand\ignore[1]{}


\newcommand\simplescheme{simple}


\newcommand{\KDF}{\mathsf{KDF}}
\newcommand{\salt}{\mathsf{sa}}
\newcommand{\PRF}{F}
\newcommand{\subgram}{\mathsf{SG}}
\newcommand{\popdomains}{\mathcal{D}}

\newcommand{\retrieve}{\textsf{Sync}}
\newcommand{\update}{\textsf{Insert}}

\newcommand{\dictW}{\textbf{D1}\xspace}
\newcommand{\dictF}{\textbf{D2}\xspace}

\newcommand{\str}{\text{str}}
\newcommand{\calS}{{\mathcal S}}

% \newcommand{\new}[1]{\textcolor{red}{\sf #1}}
\newcommand{\new}[1]{#1}


%% ------------------------- Rahul -----------------------
\newcounter{rcnote}[section]
\newcommand{\rcthenote}{\thesection.\arabic{rcnote}}
\newcommand{\rcnote}[1]{\refstepcounter{rcnote}{\bf \textcolor{magenta}{$\ll$RC~\rcthenote: {\sf #1}$\gg$}}}

\newcounter{mrnote}[section]
\newcommand{\mrthenote}{\thesection.\arabic{mrnote}}
\newcommand{\mrnote}[1]{\refstepcounter{mrnote}{\bf \textcolor{green}{$\ll$MR~\mrthenote: {\sf #1}$\gg$}}}

\newcounter{fknote}[section]
\newcommand{\fkthenote}{\thesection.\arabic{fknote}}
\newcommand{\fknote}[1]{\refstepcounter{fknote}{\bf \textcolor{blue}{$\ll$FK~\fkthenote: {\sf #1}$\gg$}}}

\newcounter{anote}[section]
\newcommand{\ajthenote}{\thesection.\arabic{anote}}
\newcommand{\anote}[1]{\refstepcounter{anote}{\bf \textcolor{cyan}{$\ll$AJ~\ajthenote: {\sf #1}$\gg$}}}



\newcommand{\mytab}{\hspace*{.4cm}}
\def\half{{1\over 2}}
\newcommand{\NT}[1]{\texttt{#1}}
\DeclareMathSymbol{\mlq}{\mathord}{operators}{``}
\DeclareMathSymbol{\mrq}{\mathord}{operators}{`'}
\newcommand{\calO}{{\mathcal O}}
\newcommand{\calA}{{\mathcal A}}
\newcommand{\kamfplus}{Kamouflage\textbf{+}\xspace}
% \newcommand{\genfrom}[1]{\;{\stackrel{\,#1}{\leftarrow}}\;}
\newcommand{\genfrom}[1]{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle#1$}}}\:}}
%\newcommand{\genfrom}[1]{\;\leftarrow{\tiny \$} #1\;}
\newcommand{\twopartdef}[4]
{
  \left\{
    \begin{array}{ll}
      #1 & \mbox{if } #2 \\[4pt]
      #3 & #4
      \end{array}
      \right.
}
\newcommand{\threepartdef}[6]
{
  \left\{
    \begin{array}{lll}
      #1 & \mbox{if } #2 \\
      #3 & \mbox{if } #4 \\
      #5 & \mbox{if } #6
      \end{array}
      \right.
}

\newcommand{\gt}[1]{\gamma_{#1,\maxdist}}
\newcommand{\gmt}[2]{\gamma_{#1,#2}}
\def\nh{\ensuremath{N}}
\def\ball{\ensuremath{B}}
\def\anh{\ensuremath{\tilde{N}_k}}
% \newcommand{\nh}[2]{{N_{#1}(#2)}}

\newcommand{\ballsizet}[1]{{\beta_{#1,\maxdist}}}
\newcommand{\ballsize}[2]{{\beta_{#1,#2}}}
\newcommand{\rh}[2]{{\bf R}_{#1, #2}}
\newcommand{\rhf}[2]{R_{f, \gamma}}
\newcommand{\realm}{{m}}
% \newcommand{\inputm}{{\tilde{m}}}
\newcommand{\lmid}{\ell_{\realm, m'}}
\newcommand{\cipherlength}{n}
\renewcommand{\SS}{\textsf{SS}}
\newcommand{\Rec}{\textsf{Rec}\xspace}
\newcommand{\rec}{\textsf{rec}\xspace}
\newcommand{\Rep}{\textsf{Rep}\xspace}
\newcommand{\Gen}{\textsf{Gen}}
\newcommand{\dis}{\textsf{dis}}

\def\chk{\textnormal{\textsf{Chk}}\xspace}
\def\reg{\textnormal{\textsf{Reg}}\xspace}
\def\exchk{\textnormal{\textsf{ExChk}}\xspace}
\def\adpchk{\textnormal{\textsf{AdpChk}}\xspace}
\def\RKROR{\textnormal{MKROR}\xspace}
\def\SRKROR{\textnormal{SKROR}\xspace}
\def\ROR{\textnormal{ROR}\xspace}
\def\ROBUST{\textnormal{ROB}\xspace}
\def\OFFDIST{\textnormal{OFFDIST}\xspace}
\def\POFFDIST{\overline{\textnormal{OFFDIST}}\xspace}
\def\OFFGUESS{\textnormal{OFFGUESS}\xspace}
\def\ONGUESS{\overline{\textnormal{ONGUESS}}\xspace}
\def\ONATTACK{\textnormal{ONATTACK}\xspace}
\def\adp{\ensuremath{\Pi\xspace}}
\def\Check{\textnormal{\textsf{Checker}}}
\def\CheckPtxt{\textnormal{\textsf{PChecker}}}
\def\trans{\textnormal{\ensuremath{T}}}
\def\transgen{\textnormal{\ensuremath{\mathcal{T}}}}
\def\pke{\ensuremath{\mathcal{E}}}
\def\pkenc{\ensuremath{\pke^{\mathrm{enc}}}}
\def\pkdec{\ensuremath{\pke^{\mathrm{dec}}}}
\def\sH{\ensuremath\mathrm{H}^s}
\def\H{\ensuremath{\mathsf{H}}\xspace}
\def\T{\ensuremath{\mathsf{T}}\xspace}
\def\W{\ensuremath{\mathsf{W}}\xspace}
\def\F{\ensuremath{\mathsf{F}}\xspace}
\def\ret{\ensuremath{\mathrm{return}}\xspace}
\def\cs{\ensuremath{t}} % Cache Size
\def\waitlen{\ensuremath{\omega}\xspace} %waitlist size
\newcommand{\M}{{\mathcal{M}}}
\newcommand{\ent}{{\bf H}}
\newcommand{\Hfuzzy}{{\mathrm{H}}^{\rm fuzz}}
\newcommand{\Hminfuzzy}{{\mathrm{H}}^{{\rm{fuzz}}}_{t,\infty}}
\newcommand{\Hpfuzzy}{{\mathrm{H}}^{{\rm{pfuzz}}}}
\newcommand{\Hinf}{{\bf H}^{{\rm \min}}_{\infty}}
\newcommand{\Hminpfuzzy}{{\bf H}^{{\rm pfuzz}}_{t,\infty}}


\def\sa{{\sf sa}}
\def\err{{\varepsilon}}%^{(e)}}}
\newcommand{\dist}{\mathcmd{p}}
\newcommand{\distest}{\hat{\mathcmd{p}}}
\newcommand{\distvec}{\mathbf{\dist}}
\newcommand{\distvecest}{\hat{\mathbf{p}}}
\newcommand{\w}{{w}}
\newcommand{\wnew}{\tilde{w}}
\newcommand{\m}{{w}}
\newcommand{\mnew}{{\tilde{m}}}
\newcommand{\mspacevec}{\mathcmd{\mathbf{W}}}
\newcommand{\mvec}{\mathcmd{\mathbf{\m}}}
\newcommand{\mvecss}[1]{\mvec_1\ldots\mvec_{#1}}
\renewcommand{\mspace}{\mathcmd{W}}
\newcommand{\mspacebot}{{\mspace}_\bot}

\newcommand{\similar}{\mathrm{sim}}
\newcommand{\similarvec}{\mathrm{\mathbf{sim}}}

\def \mvecnew{{\tilde{\mvec}}}
\newcommand{\mvecnewss}[1]{\mvecnew_1\ldots\mvecnew_{#1}}

\DeclareDocumentCommand{\edist}{o o}{
  \ensuremath{
    \IfNoValueTF{#1}{{d}}{{\sf d}(#1,#2)}
  }
}

\newcommand{\utilinc}{\mu}
\newcommand{\secloss}{\Delta}
\newcommand{\seclossg}{\Delta^\textnormal{greedy}}
\newcommand{\seclosso}{\Delta}
%\newcommand{\maxlambda}{\lambda^*}
%\newcommand{\maxfuzzlambda}{\tilde{\lambda}^*}
\newcommand{\fuzzlambda}{\lambda^\textnormal{fuzzy}}
\newcommand{\greedylambda}{\lambda^\textnormal{greedy}}
\newcommand{\greedylambdaon}{\tilde{\lambda}^\mathrm{on}}
\newcommand{\greedylambdaoff}{\tilde{\lambda}^\mathrm{off}}
\newcommand{\seclosson}{\secloss^\mathrm{on}}
\newcommand{\seclossoff}{\secloss^\mathrm{off}}
\def \edit {\ensuremath{e}}
\newcommand\error{e}
\newcommand\tab[1][1cm]{\hspace*{#1}}

\newcommand{\mathcmd}[1]{\ensuremath{#1}\xspace} % to use a command both in math mode and non-math mode
\newcommand{\minentropy}[1]{\ensuremath{\operatorname{H_\infty}\olrk{#1}}}
\newcommand{\fuzzyminentropy}[1]{\ensuremath{\operatorname{H^{fuzz}_{\maxdist, \infty}}\olrk{#1}}}
\providecommand{\condminentropy}[2]{\ensuremath{\operatorname{\tilde{H}_\infty}\olrk{#1|#2}}}
\newcommand{\s}{\mathcmd{s}}
\newcommand{\typo}{\mathcmd{\tilde{\m}}}
\newcommand{\typoj}[1]{\ensuremath{(\typo_{#1}, j_{#1})}}
\newcommand\typojprime[1]{{(\typo_{#1}, j'_{#1})}}
\renewcommand\contrib[2]{\mathsf{cont}\left[{#1}/{#2}\right]}
\def\typovec{\ensuremath{\{\typo_i\}_{i=1}}}
\def\opttypovec{\ensuremath{\{\typo^*_i\}_{i=1}}}
\def\slotguess{\textsf{SlotGuess}}
\def\typodist{\ensuremath{\tau_\pw}}
\def\cachedtypodist{\ensuremath{{\tilde{\tau}}_{\pw}}}
\def\typodistest{\ensuremath{{\hat{\tau}}_{\pw}}}
\def\incache{T_\pw}
\newcommand{\fuzzylambda}{\ensuremath{\lambda^{\mathrm{fuzzy}}}}
%\newcommand{\errorprob}[2]{\mathcmd{\tau_{#1}({#2})}}
\newcommand{\errordist}{\mathcmd{\tau}}
\newcommand{\famdist}{\mathcmd{\mathcal{W}}}
\def\guessw{\ensuremath{W}}
\newcommand{\precdist}{W}
\newcommand{\entdef}{Z}
\newcommand{\PW}{\mathcmd{\mathcal{W}}}
\newcommand{\cachedom}{\mathcmd{\mathcal{S}}}
\newcommand{\supp}{\mbox{supp}}
\newcommand{\olrk}[1]{\ifx\nursymbol#1\else\!\!\mskip4.5mu plus 0.5mu\left(\mskip0.5mu plus0.5mu #1\mskip1.5mu plus0.5mu \right)\fi}

\newcommand{\errorprob}[1]{\mathcmd{\tau_{#1}}}
\newcommand{\errorpr}[2]{\mathcmd{\errorprob{#1}{(#2)}}}
\newcommand{\Expectation}{\mathop{\mathbb E}}
\newcommand{\hash}[2]{\mathcmd{F(#1, #2)}}
\newcommand{\hashj}[3]{\mathcmd{F_{#3}(#1, #2)}}
\newcommand{\rhh}{\mathcmd{y}}
\newcommand{\x}{\mathcmd{x}}
\newcommand{\range}{\mathcmd{R}}
\newcommand{\lmm}{\mathcmd{l_\w}}
\newcommand{\rmm}{\mathcmd{r_\w}}
\newcommand{\conflict}[2]{\mathcmd{C_{#1, #2}}}
\newcommand{\Probsub}[2]{{\Pr_{#1}\left[\,{#2}\,\right]}}
\newcommand{\Condprobsub}[3]{{\Pr}_{#1}\left[\: #2\:\left|\right.\:#3\:\right]}
\newcommand{\wmid}{l_{\w, \w^\prime}}
\newcommand{\realhash}{\mathcmd{z}}
\newcommand{\collhash}{\mathcmd{z^\prime}}
\newcommand{\floor}[1]{\left \lfloor #1 \right \rfloor }
\newcommand{\ceiling}[1]{\left \lceil #1 \right \rceil }
\newcommand{\interval}{I}
% \newcommand{\p}[2]{p_{#1}(#2)}
\newcommand{\ssketch}{\mathcmd{\mathsf{S}}}
\newcommand{\tsketch}{\mathcmd{\msgsettingsym\mathsf{S}}}
\newcommand{\trivsketch}{\mathcmd{\tsketch_{\emptystr}}}
\newcommand{\WREC}{\mathcmd{\pcnotionstyle{W\pcmathhyphen{}REC}}}
\newcommand{\AREC}{\mathcmd{\pcnotionstyle{A\pcmathhyphen{}REC}}}
\newcommand{\WUTIL}{\mathcmd{\pcnotionstyle{W\pcmathhyphen{}UTIL}}}
\newcommand{\AUTIL}{\mathcmd{\pcnotionstyle{A\pcmathhyphen{}UTIL}}}
\newcommand{\indexset}{I}
\newcommand{\topset}{Z_1^*}
\newcommand{\cachedist}{T}
\newcommand{\pwdis}{R}
\newcommand{\onbudget}{q}
\newcommand{\blacklist}{\textsf{B}}
\newcommand{\blacklistlen}{\alpha}
\newcommand{\plaintextstate}{\bar{\state}}
\newcommand{\typocutoff}{\delta}
\newcommand{\plfuprob}{\ensuremath{\nu}}

\def\ballweight{\ensuremath{e_{\tilde{\tau}}}}
\newcommand{\Adv}{\textnormal{\textsf{Adv}}}
\newcommand{\AdvOFFLINE}[1]{\Adv^{\footnotesize\textnormal{\textrm{offdist}}}_{\footnotesize #1}}
\newcommand{\AdvOFFLINEP}[1]{\Adv^{\overline{\footnotesize\textnormal{\textrm{{offdist}}}}}_{\footnotesize #1}}
\newcommand{\AdvOFFGUESS}[1]{\Adv^{\footnotesize\textnormal{\textrm{offguess}}}_{\footnotesize #1}}
\newcommand{\AdvONGUESS}[1]{\Adv^{{\footnotesize\textnormal{\textrm{onguess}}}}_{\footnotesize #1}}
\newcommand{\AdvONATTACK}[1]{\Adv^{\footnotesize\textnormal{\textrm{onattack}}}_{\footnotesize #1}}
\newcommand{\AdvRKROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{mk-ror}}}_{\footnotesize #1}}
\newcommand{\AdvSRKROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{sk-ror}}}_{\footnotesize #1}}
\newcommand{\AdvROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{ror}}}_{\footnotesize #1}}
\newcommand{\AdvROBUST}[1]{\Adv^{\footnotesize\textnormal{\textrm{rob}}}_{\footnotesize #1}}

\newcommand{\advantage}[3]{\pcnotionstyle{\Adv}^{#1}_{#2}(#3)}
\newcommand{\neighbourhood}[2]{N_{#1}({#2})}
\newcommand{\rhhdist}{Y}
\newcommand{\fullerhash}{z}
\newcommand{\errorball}[2]{{B}^{\errordist}_{#1}(#2)}
\newcommand{\f}{f}
\newcommand{\pwmaxlen}{\ell}
\newcommand{\indexi}{i}
\newcommand{\indexq}{q}
\newcommand{\indexx}{x}
\newcommand{\replace}{\textsf{replace}}
\newcommand{\vecca}{\vecc{a}}
\newcommand{\veccb}{\vecc{b}}
\newcommand{\veccv}{\vecc{v}}
\newcommand{\coins}{r}
\renewcommand{\state}{\ensuremath{\mathsf{s}}}
\newcommand{\win}{\mathsf{win}}
\newcommand{\Chk}{\textsf{Chk}}
\newcommand{\PChk}{\textsf{PChk}}
\newcommand{\indexh}{h}
\newcommand{\randomZ}{Z}
\newcommand{\Cache}{\textnormal{\textsf{Cache}}}
\newcommand{\WarmupCache}{\textnormal{\textsf{WarmupCache}}}
\newcommand{\CacheUpdate}{\textnormal{\textsf{CacheUpdt}}}
\newcommand{\CacheInit}{\textnormal{\textsf{CacheInit}}}
\newcommand{\cachestate}{\ensuremath{\mathtt{S}}\xspace}
\newcommand{\cachestatelen}{\ensuremath{\sigma}\xspace}
\newcommand{\CacheLRU}{\textnormal{\textsf{CacheLRU}}}
\newcommand{\CacheLRUUpdate}{\textnormal{\textsf{UpdateLRU}}}
\newcommand{\CacheLRUInit}{\textnormal{\textsf{InitLRU}}}


\newcommand{\zxcvbn}{\textnormal{\textsf{zxcvbn}}\xspace}
\newcommand{\bad}{\textnormal{\textsf{bad}}}
\newcommand{\wait}{z}
\newcommand{\PKE}{\textnormal{\textsf{PKE}}}
\newcommand{\pkegen}{\mathcal{K}}
\newcommand{\pkeenc}{\mathcal{E}}
\newcommand{\pkedec}{\mathcal{D}}
\newcommand{\pkectxtspace}{\mathcal{C}_{\pkeenc}}
\newcommand{\pk}{{pk}}
\newcommand{\sk}{{sk}}
\newcommand{\PBE}{\textnormal{\textsf{PBE}}}
\newcommand{\utility}{\textsf{Utility}}

\newcommand{\skegen}{\ensuremath{\mathsf{K}}}
\newcommand{\skeenc}{\ensuremath{\mathsf{E}}}
\newcommand{\skedec}{\ensuremath{\mathsf{D}}}
\newcommand{\skectxtspace}{\ensuremath{\mathcal{C}_{\skeenc}}}
\newcommand{\ske}{\textnormal{\textsf{SKE}}}
\newcommand{\SE}{\textnormal{\textsf{SE}}}
\newcommand{\sekg}{\mathcal{K}}
\newcommand{\seenc}{\mathcal{E}}
\newcommand{\sedec}{\mathcal{D}}
\newcommand{\saltlen}{{\ell_{\mathrm{salt}}}}

\newcommand{\skk}{\textnormal{\textsf{k}}}
\newcommand{\cipherske}{{c}}
\newcommand{\cipherpke}{{c}}
\newcommand{\SH}{\textnormal{\textsf{SH}}}
\newcommand{\FH}{\textnormal{\textsf{H}}}
\newcommand{\counter}{\textnormal{\textsf{Count}}}
\newcommand{\indexp}{p}
\newcommand{\ciphertextspace}{\mathcal{C}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\indexr}{r}
\newcommand{\vecc}[1]{\mathbf{#1}}
\newcommand{\sawait}{\overline{\sa}}
\newcommand{\skkwait}{\overline{\skk}}
\newcommand{\hwait}{\overline{\indexh}}
\newcommand{\randomY}{Y}
\newcommand{\indexm}{m}
\newcommand{\hashtable}[1]{H[#1]}
\newcommand{\SHlen}{k_1}
\newcommand{\FHlen}{k_2}
\newcommand{\valid}{\textnormal{\textsf{valid}}}
\newcommand{\skepsilon}{\epsilon_{ske}}
\newcommand{\pkepsilon}{\epsilon_{pke}}
\newcommand{\hybindex}{j}

\newcommand{\DL}{\textnormal{DL}}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\indicator}{\mathbb{I}}
\newcommand{\cipherspace}{\mathcal{C}}
\newcommand{\pkemsgspace}{\mathcal{M}_\pkeenc}

\newcommand{\pkecipher}{c}
\newcommand{\skecipher}{{c}}
\newcommand{\pkemsg}{m}
\newcommand{\skemsg}{{m}}
\newcommand{\skemsgspace}{ \msgspace_{\skeenc}}
\newcommand{\upperb}{\alpha}

\newcommand{\ffbox}[1]{
   \setlength{\fboxsep}{-1\fboxrule}
   \fbox{\hspace{1.2pt}\strut#1\hspace{1.2pt}}}


\newcommand{\statespace}{S}
\newcommand{\targuess}{\textsf{TarGuess}}
\newcommand{\untarguess}{\textsf{UnTarGuess}}

\newcommand{\accept}{\texttt{accept}}
\newcommand{\reject}{\texttt{reject}}
\newcommand{\threshold}{\ensuremath{\tau}}
\newcommand{\clfthreshold}{\ensuremath{\theta}}
\newcommand{\far}{\ensuremath{\alpha}}
\newcommand{\frr}{\ensuremath{\beta}}
\newcommand{\fpr}{\ensuremath{\nu}}
\newcommand{\fnr}{\ensuremath{\gamma}}
\newcommand{\FPR}{\textrm{FPR}}
\newcommand{\FNR}{\textrm{FNR}}


\newcommand{\matchalgo}{\mathcal{L}}
\newcommand{\matchalgovec}{\mathcal{\mathbf{L}}_\sslen}
\def \score {\theta}
\newcommand{\indexjvec}{\ensuremath{\mathcmd{\mathbf{j}}\xspace}}
\def\k{k}
\newcommand{\add}{\funcfont{Add}}
\newcommand{\accuracy}{\funcfont{Accuracy}}
\def\acc{\delta}
\def \MS {\funcfont{MS}}
\def \MRec {\funcfont{MRec}}
\newcommand \MSt{\MS^{\matchalgo}_\sslen}
\newcommand \MRect{\MRec^{\matchalgo}_\sslen}
\def \nmatches {\ensuremath{l}}
\def \D{D}
\def \Dmod{\tilde{D}}
\def \mlen{n}
\def \sslen{t}
\def \secret{s}
\def \secretvec{\mathbf{s}}
\newcommand{\sketch}{{\funcfont{sketch}}}
\newcommand{\sketchval}{v}
\def \recover{\funcfont{recover}}
\def \verify{\funcfont{verify}}
\def \q{q}
\def\fp{\alpha}
\def\fn{\beta}
\def\tp{\gamma}
\newcommand{\one}{\ensuremath{\mathbbm{1}}}
\newcommand{\seclen}{\ell}
\newcommand{\Overify}{{\mathcal{O}_\funcfont{vrfy}}}
\newcommand{\Omatch}{\mathcal{O}_\funcfont{match}}
\newcommand{\ith}[2]{#1_{#2}}
\newcommand{\jth}[2]{#1^{#2}}
\newcommand{\mspacei}{\ith{\mspace}{i}}
\newcommand{\errori}{\ith{\error}{i}}
\newcommand{\matchalgoi}{\ith{\matchalgo}{i}}
\newcommand{\mvecbar}{\overline{\mvec}}
\newcommand{\mvectilde}{\tilde{\mvec}}
\newcommand{\angbrac}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\clf}{\mathcal{C}}
\newcommand{\clft}{\clf_\sslen}
\newcommand{\clfest}{\mathcal{\hat{\clf}}}
\newcommand{\clfq}[1]{{\clf^q_{#1}}}
\newcommand{\nclf}{r}
\newcommand{\oclf}{\omega}
\newcommand{\biosketch}{\funcfont{TenSketch}\xspace}
\newcommand{\tensketch}{\funcfont{TenSketch}\xspace}

\newcommand{\hvec}{\mathbf{h}}
\newcommand{\insertr}{\mathsf{insert{\scriptstyle\$}}}
\newcommand{\dbmsg}{\ensuremath{\mathcal{F}}}
\newcommand{\dbmsgs}{\ensuremath{\{\dbmsg_i\}}}
\newcommand{\dbid}{\mathcal{I}}
\newcommand{\db}{\ensuremath{D}}
% \newcommand{\dbs}{\ensuremath(\dbid,\{\dbmsg_i\})}
\newcommand{\dbs}{\ensuremath(\dbid,\dbmsg)}
\newcommand{\dbsprime}{\ensuremath(\dbid',\dbmsg')}
\newcommand{\dbsize}{N}
\def \dblen{N}
\def\mhat{\hat{\mvec}}
\def\findmatches{\funcfont{\footnotesize FindMatches$^{\matchalgo}$}}
\newcommand{\setss}[1]{\SS^\Delta_{#1}}
\newcommand{\setrec}[1]{\Rec^\Delta_{#1}}
\newcommand{\setsst}{\setss{\sslen}}
\newcommand{\setrect}{\setrec{\sslen}}
\newcommand{\costs}{{c_s}}
\newcommand{\costc}{{c_c}}
\NewDocumentCommand{\indseq}{ O{1} O{r} }{{#1}\ldots {#2}}
\newcommand{\seq}[2]{{{#1}_1,\ldots,{#1}_{#2}}}
\newcommand{\relu}{\funcfont{ReLu}}
\newcommand{\fcrelu}[1]{\funcfont{FC}_{\relu}^{#1}}
\newcommand{\gencliq}{\funcfont{GenTupIncr}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> figures/relro-code.tex <==
\begin{figure*}[t!]
  \centering
  \begin{subfigure}[b]{0.28\textwidth}
    \centering
\begin{lstlisting}[language={[x86masm]Assembler},basicstyle={\scriptsize\ttfamily},numberstyle=\scriptsize,xleftmargin=5mm,deletekeywords={df,}]
; function start
b0: push   rbp        ; 1
b1: lea    rax,[rip+0x36d8b8]
b8: lea    rbp,[rdi+0x50]
bc: push   rbx        ; 2
bd: lea    rbx,[rdi+0xb0]
c4: sub    rsp,0x8    ; 3
c8: mov    QWORD PTR [rdi],rax
cb: nop    DWORD PTR [rax]
d0: sub    rbx,0x18
d4: mov    rdi, QWORD PTR [rbx]
d7: call   3d5c0 <qfree@plt>
dc: cmp    rbp,rbx
df: jne    45fd0 <main+0x55e0>
e1: add    rsp,0x8    ; 4
e5: pop    rbx        ; 5
e6: pop    rbp        ; 6
e7: ret
; function end
\end{lstlisting}
    \caption{Assembly code}
    \label{fig:sub1}
  \end{subfigure}
\end{figure*}

==> images/mainflow.tex <==
% \section{Diagrammatic view of Multisketch operations}\label{app:mainflow}  

% A user registers with a user id $\u$ and a vector of biometric templates
% $\mvec=\mvecss{\mlen}$. Multisketch uses two databases $\dbid$ and $\dbmsg$\@,
% where $\dbid$ contains user id $\u$ and the corresponding helper data
% $\sketchval$, and $\dbmsg$ contains the random permutation of the templates
% registered so far. Highlighted are the entries corresponding to a user $\u_4$
% with templates $\mvec_4=\mvec_{41}\ldots\mvec_{4\mlen}$.% and helper
%     % data $\sketchval_4$.
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
    >=stealth,
    node distance=2cm,
    database/.style={
      cylinder,
      cylinder uses custom fill,
      cylinder body fill=black!25!white,
      cylinder end fill=black!25!white,
      shape border rotate=90,
      aspect=0.25,
      minimum width=2em,
      minimum height=2em,
      draw
    },
    func/.style={
      rectangle,
      fill=red!25!white,
      minimum width=1cm,
      minimum height=1em,
      draw
    },
    cell/.style={
      rectangle,
      draw=black!50!white
    }
    ]
    \node (user) at (0, 0) {User};
    \node[func, right of=user, right=-1.1em, above=3em] (msketch) {$\MS$}; 
    \draw[below of=msketch, dashed, anchor=west] (.85,0.55) rectangle (5.9,-1.2); 
    \node[func, below of=msketch, anchor=east, below=1.95cm,fill=red!10!white,dashed] (mrecover) {$\MRec$};
    % \node[database, right of=user, anchor=south, above=1em, right=2cm] (db1) {$\dbid$};
    \matrix (db1) [right of=user, anchor=south, below=2pt, right=-0.1cm, 
    matrix of math nodes,
    column sep = -\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}}, 
    column 2/.style={nodes={cell}}, 
    anchor=west] {
      \u_1 & \sketchval_1\\
      \u_2 & \sketchval_2\\
      \u_3 & \sketchval_3\\
      |[draw,fill=blue!20]|\u_4 & |[draw,fill=blue!20]|\sketchval_4\\
    };
    \node[left of=db1, anchor=east,right=1.1cm] {$\dbid$};
    \matrix (db2) [right of=db1, left=25pt, matrix of math nodes,
    column sep = 2\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}},
    column 2/.style={nodes={cell}}, 
    column 3/.style={nodes={cell}}, 
    column 4/.style={nodes={cell}}, 
    column 5/.style={nodes={cell}}, 
    anchor=west] {
      \mvec_{21} &\mvec_{12} & |[draw,fill=blue!20]|\mvec_{43} &  & \mvec_{3\mlen} \\
      |[draw,fill=blue!20]|\mvec_{41} &\mvec_{32} & \mvec_{33} & |[draw=white]|\ldots & \mvec_{2\mlen} \\
      \mvec_{11} &|[draw,fill=blue!20]|\mvec_{42} & \mvec_{23} &  & \mvec_{1\mlen} \\
      \mvec_{31} &\mvec_{22} & \mvec_{13} & & |[draw,fill=blue!20]|\mvec_{4\mlen} \\
    };
    \node[left of=db2, left=-4pt] {$\dbmsg$};

    % \node[database,right of=db1] (db2) {$\dbmsg$};
    \node[func,below of=db1,anchor=north,above=8pt,left=8pt] (gu) {GetUser};
    \node[func,right of=gu,anchor=east,right=-5pt] (fm) {FindMatches};
    \node[func,below of=db1,anchor=east,below=2em,right=-3pt] (recover) {Recover};

    \draw[->,blue!50,thick] (user.north) |- node[black,near end,above]{$u, \mvec$} node[black,near end,below,font=\small]{register} 
    (msketch.west);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$u, \sketchval$} (db1);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$\mvec$} (db2);

    \draw[->,blue!50,thick] (user.south) |- ++(1,-0.9) node[black,near end,above]{$u, \mvectilde$} node[black,near end,below,font=\small]{login}   -| node[black,left,near end]{$u$}
    (gu.north);
    \draw[->,blue!50,thick] (user.south) |- ++(0,-0.9)  -- ++(3.1,0) |- node[black,near end, above]{$\mvectilde$}
    (fm.west);
    \draw[->,blue!50,thick] (db1.south) |- node[black,near end,above]{} (gu.east);
    \draw[->,blue!50,thick] (db2.south) |- node[black,near end,above]{} (fm.east);
    \draw[->,blue!50,thick] (gu.south) |- node[black,near end,above]{$\sketchval$} (recover.west);
    \draw[->,blue!50,thick] (fm.south) |- node[black,near end,above]{$\mvec'$} (recover.east);    
    \draw[->,blue!50,line width=2pt] (recover.south) -- node[black,near end,right]{$\mvec$ or $\bot$} ++(0, -0.65);
  \end{tikzpicture}
  % \rcnote{Rough sketch of the flow of the \biosketch.} 
  \caption{Diagram of multisketch as a part of an authentication service. 
  }
  \label{fig:mainflow}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}

\jun{This should not be a separate section; The contents should be 
scattered to the previous sections.}

% We reuse 6 spiders from FIRMADYNE and rewrite spiders for all the other vendors listed in Table~\ref{tab:vendors}.  
% \subsection{Firmware Unpacking}
% We implement extraction script based on BINWALK and FIRMADYNE. BINWALK occasionally omit many kernels because BINLWAK apply Linux version string check which lead to many failures of recognizing valid Linux kernel. We fix this problem by removing the unnecessary check in BINWALK. In case of filesystem extraction, FIRMADYNE determines UNIX-like root file-system based on heuristics which require UNIX-like filesystem must contains sufficient UNIX-like sub-directory including bin, etc, dev, home, lib, mnt, opt, root, run, sbin, tmp, usr and var. We extend the list of the UNIX-like sub-directory with share, sys and proc since \studentfix{XXX}. FIRMADYNE provides the functionality to extract filesystem and kernel simultaneously, however, we decide to separate the extraction process because extract filesystem and kernel together is more likely to trigger the early termination threshold which may lead to unexpected omission. To achieve better runtime performance, we slightly change the default thresholds used in FIRMADYNE, reducing recursive breath threshold from 5 to 4 and recursive depth threshold from 3 to 2 for two reasons. First, we believe the default threshold is used as extracting filesystem and kernel simultaneously. It is more reasonable to tighten the thresholds as we separate the extraction process. Second, based on our empirical observation, both Linux kernel and root file-system are most likely to be placed in the first-level content in firmware images. Terminate recursive extraction at lower depth has little influence on the result but save much more execution time. 
% Kernel is an important component of an IoT device software which can be identified from the firmware image. As FIRMADYNE does not support incomplete, recursively structured and non-Linux-based firmware images, we categorize all the images failed to be extracted as unknown. 



==> note.tex <==

%Definition of firmware

%The term ”firmware” has been coined by Ascher Opler in
%in a 1967 Datamation article. His definition of firmware
%as a glue microcode layer between the CPU instruction set
%and the actual hardware has since been superseded, and the
%IEEE Standard Glossary of Software Engineering Terminology, Std %610.12-1990, defines firmware today as follows:
%The combination of a hardware device and computer instructions and data %that reside as readonly software on that device.
%Notes: (1) This term is sometimes used to refer
%only to the hardware device or only to the computer instructions or %data, but these meanings
%are deprecated.
%Notes: (2) The confusion surrounding this term
%has led some to suggest that it be avoided altogether.
%For the sake of simplicity we will deviate from this definition in that %we call the set of all code running on the hardware’s processor %(machine code and virtual machine code)
%the firmware of this device.

==> tables/arch-elfmeasure.tex <==
\begin{table}[t]
  \centering
  \caption{Analysis of Binary Hardening Measure Cross Architecture}
  \label{tab:arch-result}
  \scriptsize
  \begin{tabular}{ c| c| c| c| c| c| c}
    \hline\hline
    \multirow{2}{*}{\textbf{Arch}} & \multirow{2}{*}{\textbf{ELF}} & \multirow{2}{*}{\textbf{PIE}} & \multirow{2}{*}{\textbf{NX}} & \multirow{2}{*}{\textbf{Canary}} & \multirow{2}{*}{\textbf{Fortify}} & \multirow{2}{*}{\textbf{RELRO}}  \\
    & & &  & &  \\ \cline{1-7}
    aarch64 & 53.7k & 12.8 & \cellcolor{lightgray}{99.8} & 41.1 & 40.4 & \cellcolor{lightgray}{62.2} \\ \hline
    ppc & 54.4k & 10.7 & 92.8 & 27.7 & 27.5 & 0.4  \\ \hline
    x86-64 & 53.6k & 13.8 & 99.6 & 44.4 & \cellcolor{lightgray}{44.4} & 60.2 \\ \hline
    x86 & 331.7k & \cellcolor{lightgray}{8.3} & 99.2 & \cellcolor{lightgray}{76.1} & 5.8 & 9.4 \\ \hline
    arm & 1129.1k & 13.7 & 97.2 & 30.6 & 29.3 & 13.7 \\ \hline
    mips & 815.1k & 8.6 & 27.0 & 0.8 & 5.3 & 0.001  \\ \hline 
    Other & 0.8k & 13.4 & 73.7 & 0.5 & 0.4 & 23.3 \\ \hline
    \hline
  \end{tabular}
  \vspace{-1.5em}
\end{table}

==> tables/config-result-tmp.tex <==
\begin{table*}[t!]
  \centering
  \caption{Analysis of Configuration Files}
  \label{tab:config-result}
  \scriptsize
  \begin{tabular}{ c c c c c c c}
    \hline\hline
    \textbf{Vendors} & \textbf{Config File} & \textbf{Stack Canary} & \textbf{Fortify Source} & \textbf{Usercopy} & \textbf{Kernel RWX} & \textbf{Others}\\ \hline
    \textbf{linksys} &  24 & 8  & 0 & 0 & 0 & 0      \\  \hline
    \textbf{netcore} &  1 & 0  & 0 & 0 & 0 & 0      \\  \hline
    \textbf{netgear} &  269 & 44  & 0 & 0 & 2 & 0      \\  \hline
    \textbf{openwrt} &  9 & 9  & 4 & 3 & 5 & 0      \\  \hline
    \textbf{polycom} &  16 & 0  & 0 & 0 & 0 & 0      \\  \hline
    \textbf{supermirco} &  9 & 0  & 0 & 0 & 0 & 0      \\  \hline
    \textbf{tplink-en} &  43 & 8  & 0 & 0 & 0 & 0      \\  \hline
    \textbf{tplink-zh} &  53 & 2  & 0 & 0 & 0 & 0      \\  \hline
    \textbf{trendnet} &  3 & 0  & 0 & 0 & 0 & 0      \\  \hline
    \textbf{phicom} &  1 & 0  & 0 & 0 & 0 & 0      \\  \hline
    \textbf{Tot} &  437 & 71  & 4 & 3 & 7 & 0      \\  \hline
    \hline
  \end{tabular}
  \vspace{-1.5em}
\end{table*}

==> tables/elfmeasure_tmp.tex <==
\begin{table*}[t]
  \centering
  \caption{Analysis of Binary Hardening Measure}
  \label{tab:mitigation-result}
  \scriptsize
  \begin{tabular}{ c| c| c| c| c| c| c| c| c| c| c| c| c| c| c| c}
    \hline\hline
    \multirow{2}{*}{\textbf{Vendors}} & \multirow{2}{*}{\textbf{PIE}} & \multicolumn{3}{c|}{\textbf{Non-Exec Stack}} & \multicolumn{3}{c|}{\textbf{Stack Canary}} & \multicolumn{3}{c|}{\textbf{Fortify Source}} & \multicolumn{3}{c|}{\textbf{RELRO}}  & \multirow{2}{*}{\textbf{Avg}} & \multirow{2}{*}{\textbf{ELF}}\\ \cline{3-14}
    & & our & PWN & Sec & our & PWN & Sec & our & PWN & Sec & our & PWN & Sec & \\ \cline{1-16}
    \textbf{aarch64} & 60.1 & 99.8 & & & 41.1 & & & 40.4 & & & 62.2 & & & 60.7 & 53702\\ \hline
    \textbf{ppc} & 58.2 & 92.8 & & & 27.7 & & & 27.5 & & & 0.4 & & & 41.3 & 54363\\ \hline
    \textbf{x86-64} & 60.8 & 99.6 & & & 44.4 & & & 44.4 & & & 60.2 & & & 61.9 & 535901\\ \hline
    \textbf{x86} & 62.5 & 99.2 & & & 76.1 & & & 5.8 & & & 9.4 & & & 50.6 & 331702\\ \hline
    \textbf{arm} & 62.2 & 97.2 &  & & 30.6 & & & 29.3 & & & 13.7 & & & 46.6 & 1129065\\ \hline
    \textbf{mips} & 60.0 & 27.0 & & & 0.8 & & & 5.3 & & & 0.001 & & & 18.6 & 815056\\ \hline 
    \textbf{Other} & 31.0 & 73.7 & & & 0.5 & & & 0.4 & & & 23.3 & & & 25.8 & 751\\ \hline \hline
    \textbf{Actiontec} & 30.4 & 47.9 & 60.1 & & 0.5 & & & 0.5 & & & 0 & & & 15.9 & 406\\ \hline
    \textbf{ASUS} & 62.4 &  46.8 & 78.2 & & 1.3 & & &  0.05 & & & 1.3 & & & 22.4 & 273211\\ \hline
    \textbf{At\&t} & 22.1 &  10.5 & 16.9 & & 0 & & &  0 & & & 0 & & & 9.9 & 593\\ \hline
    \textbf{Clink} & 38.7 & 0.2 & 36.4  & & 0 & & &  0 & & & 0 & & & 15.1 & 782\\ \hline
    \textbf{phicomm} & 59.9 & 47.0 & 76.1 & & 0.1 & & &  0 & & & 0 & & & 21.4 & 1898\\ \hline
    \textbf{qnap} & 62.5 &  99.2 & 99.7 & & 80.1 & & &  1.4 & & & 3.1 & & & 49.3 & 295969\\ \hline
    \textbf{synology} & 62.5 & 99.5 & 99.8 & & 43.6 & & &  \textcolor{red}{43.5} & & & 36.7 & & & 57.2 & 1375420\\ \hline
    \textbf{tenda} & 50.2 & 30.2 & 60.7 & & 0.6 & & &  0.01 & & & 2.3 & & & 16.7 & 33623\\ \hline
    \textbf{digi} & 59.9 & 3.5 & 58.1 & & 0 & & &  0 & & & 0 & & & 12.7 & 1456\\ \hline
    \textbf{tm-shibby} & 71.8 & 23.2 & 76.3 & & 0.1 & & &  0 & & & 1.0 & & & 19.2 & 127824\\ \hline
    \textbf{ubiquiti} & 62.8 & 15.6 & 65.2 & & 6.7 & & &  25.0 & & & 1.0 & & & 22.2 & 204278\\ \hline
    \textbf{moxa} & 67.5 & 77.3 & 89.4 & & 39.3 & & &  35.5 & & & 15.2 & & & 47.0 & 31975\\ \hline \hline
    \textbf{360}    &  22.4 & 0  & 14.4 & 0 & 59.8 & 59.8 & 59.8 & 0 & 0 & 0 & 0 & 5.2 & 5.2 & 16.4 & 458      \\  \hline
    % \textbf{ASUS}   &  64.4\% & 64.4\%    & - & 96.45\%  & 98.5\% & 98.5\% & 0 & 0.2\% & 0.2\% & 0 & 0 & 0 & 2.08\% & 4.2\% & 4.2\% & 3563      \\  \hline
    \textbf{AVM}    &  \textcolor{red}{95.2} & 95.7 & 97.7 & 95.7 & \textcolor{red}{81.5} & 81.5 & 81.5 & 0.04 & 0.1 & 0.2 & \textcolor{red}{89.5} & 91.1 & 91.1 & \textcolor{red}{72.4} & 5064      \\  \hline
    \textbf{Belkin} &  55.4 & 8.6  & 53.6 & 12.0 & 0.2 & 0.2 & 0.2 & 1.6 & 1.6 & 2.1 & 3.8 & 5.2 & 5.2 & 13.9 & 7872      \\  \hline
    \textbf{buffalo} &  37.5 & 45.9  & 64.3 & 52.2 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 52.6 & 52.6 & 16.7 & 456      \\  \hline
    \textbf{Camius} &  50.4 & 92.1  & 94.7 & 95.2 & 11.9 & 11.9 & 11.9 & 1.3 & 1.3 & 1.3 & 0 & 12.1 & 12.1 & 31.1 & 454      \\  \hline
    \textbf{cerowrt} &  57.2 & 0  & 52.6 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 4.1 & 4.1 & 11.4 & 388      \\  \hline
    \textbf{Dlink} &  44.9 & 95.5  & 57.8 & 35.0 & 0.4 & 0.4 & 0.4 & 0.04 & 0 & 0.2 & 0.31 & 2.9 & 2.9 & 28.2 & 15907      \\  \hline
    % \textbf{gocloud} &  63.2\% &   63.2\% & - & 98.95\%  & 99.2\% & 99.2\% & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 7.2\% & 7.2\% & 899      \\  \hline
    \textbf{haxoware} &  63.7 & 0  & 57.3 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.6 & 7.1 & 7.1 & 12.9 & 157      \\  \hline
    % \textbf{hiwifi} &  49.7\% & 49.7\%    & - & 97.36\%  & 98.7\% & 98.0\% & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 92.7\% & 92.7\% & 1727      \\  \hline
    \textbf{Linksys} &  54.2 & 60.4  & 80.1 & 63.7 & 0.5 & 0.5 & 0.5 & 0.8 & 0.9 & 1.2 & 3.0 & 6.8 & 6.8 & 23.8 & 17073      \\  \hline
    \textbf{Mercury} &  63.2 & 0  & 46.3 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 6.3 & 6.3 & 12.6 & 1450      \\  \hline
    \textbf{Mikrotik} &  26.9 & 81.0  & 62.8 & 51.9 & 0.2 & 0.2 & 0.2 & 0.09 & 0 & 0.09 & 7.8 & 18.5 & 18.5 & 23.2& 4294      \\  \hline
    \textbf{Netcore} &  34.7 & 0.06  & 21.9 & 0.05 & 11.3 & 11.3 & 11.3 & 0.2 & 0.06 & 0.3 & 0 & 11.6 & 11.6 & 9.3 & 10189      \\  \hline
    \textbf{Netgear} &  47.6 & 55.9  & 73.9 & 59.1 & 2.2 & 2.2 & 2.2 & 0.5 & 0.4 &  0.6 & 4.3 & 10.3 & 10.3 & 22.1 & 173852      \\  \hline
    \textbf{openwrt} &  43.6 & \textcolor{red}{99.9}  & 99.9 & 99.1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 99.1 & 99.1 & 28.7 & 191194      \\  \hline
    % \textbf{Phicomm} &  50.9\% & 50.9\%  & - & 32.33\%  & 63.9\% & 30.5\% & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2.6\% & 2.6\% & 499      \\  \hline
    \textbf{RouterTech} &  30.6 & 0  & 18.3 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 6.1 & 25845      \\  \hline
    \textbf{Supermirco} &  57.8 & 97.8  & 98.9 & 98.9 & 19.4 & 19.4 & 19.4 & 0 & 15.4 & 15.8 & 3.2 & 13.2 & 13.2 & 35.6 & 1307      \\  \hline
    % \textbf{Tenda-en} &  50.2\% & 22.53\%  & 56.2\% & 33.7\% & 0.7\% & 0.7\% & 0.7\% & 0 & 0.1\% & 0.5\% & 1.83\% & 4.8\% & 4.8\% &   8211    \\  \hline
    % \textbf{Tenda-zh} &  60.0\% & 50.03\%  & 77.1\% & 62.0\% & 1.2\% & 1.2\% & 1.2\% & 0 & 0.04\% & 0.4\% & 3.04\% & 7.6\% & 7.6\% &  8542      \\  \hline
    \textbf{Tenvis} &  41.3 & 0  & 11.0 & 0 & 0 & 0 & 0 & 0 & 0 & 5.5 & 0 & 8.3 & 8.3 & 8.3 & 908      \\  \hline
    % \textbf{Tomato} &  71.0\% & 14.82\%  & 73.3\% & 12.6\% & 0.1\% & 0.1\% & 0.1\% & 0 & 0.4\% & 0.7\% & 0.52\% & 2.1\% & 2.1\% & 55861      \\  \hline
    \textbf{Tplink-en} &  51.3 & 36.6  & 60.7 & 30.4 & 0.5 & 0.5 & 0.5 & 0.6 & 0.7 & 0.9 & 0.9 & 9.8 & 9.8 & 18.0 & 76332     \\  \hline
    \textbf{Tplink-zh} &  61.6 & 38.7  & 70.3 & 72.8 & 2.9 & 2.9 & 2.9 & 0.1 & 0.03 & 0.2 & 0.4 & 21.0 & 21.0 & 20.7 & 65650    \\  \hline
    \textbf{Trendnet} &  50.9 & 10.1  & 48.9 & 14.8 & 0.4 & 0.4 & 0.4 & 0.05 & 0.05 & 0.3 & 0.3 & 14.2 & 14.2 &  12.4  & 15263   \\  \hline
    % \textbf{Ubiquiti} &  64.9\% & 64.9\% & - & 1.45\%  & 61.0\% & 2.5\% & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 3.3\% & 3.3\% &  9930    \\  \hline
    \textbf{Zyxel} &  34.5 & 97.3  & 98.0 & 97.9 & 1.0 & 1.0 & 1.0 & 0.9 & 0 & 1.0 & 0 & 49.1 & 49.1 & 26.7  & 804    \\  \hline
    \hline
    \textbf{STC Binary} & 0  &  33.5 & 32.9 & 31.2 & 2.0 & 0 & 0 & 0 & 0 & 0 & 0.7 & 3.2 & 3.2 &  & 2197    \\  \hline
    \hline
  \end{tabular}
  \vspace{-1.5em}
\end{table*}

==> tables/fw_date.tex <==

\begin{table*}[t!]
  \centering
  \caption{Time Spread of Download Firmware}
  \label{tab:fw_category}
  \scriptsize
  \begin{tabular}{c c c c c c c c c c c c c c|c}
    \hline\hline
    &\textbf{bf 2010} & \textbf{2011} & \textbf{2012} &\textbf{2013} &\textbf{2014} &\textbf{2015} &\textbf{2016} &\textbf{2017} &\textbf{2018} &\textbf{2019} &\textbf{2020} &\textbf{2021} &\textbf{Unavailable} &\textbf{Num}\\ \hline
    \textbf{360}        &  -    &    -      &   -       &   -   &   -   & - & - & 100\% & - &  - & - & - & - & 5\\  \hline
    \textbf{Buffalo}    &  -    & -         & -         &   -   &  -    & - & 16.7\% & - & 83.3\% & - & - & - & - & 6 \\  \hline
    \textbf{Cerowrt}    & -     &  -        &    -      & -     &   -   & 100\% & - & - & - & - & - & - & - & 2\\  \hline
    \textbf{Dlink}      & 20.0\%     &  5.1\%        &    4.6\%      & 20.6\% & 7.6\%  &  5.9\% & 6.0\% & 5.6\% & 6.5\% & 10.6\% & 7.1\% & 0.4\% & - & 1172\\  \hline
    \textbf{Gocloud}  & -  &  - &  - & -   & - & - & - & - & - & 12.5\% & 75.0\% & 12.5\% & - & 8\\  \hline
    \textbf{Linksys}  & 1.2\%     &  0.6\%        &    6.0\%      & 4.2\%     &   9.0\%   & 4.8\% & 9.6\% & 12.7\% & 17.5\% & 9.0\% & 21.7\% & 3.6\% & - & 166\\  \hline
    \textbf{Mercury}     &  -    & 17.8\%         & 16.6\%         &   11.8\%   &   12.4\%   & 13.6\% & 0.6\% & - & - & 0.6\% & - & - & - & 169 \\  \hline
    \textbf{Netcore}     &  -    & -         & -         &   -   &   -   & - & - & - & - & - & 98.8\% & 1.2\% & - & 255 \\  \hline
    \textbf{RouterTech}  & 75.0\%     &  16.7\%        &    8.3\%      & -     &   -   & - & - & - & - & - & - & - & - & 144\\  \hline
    \textbf{Tenvis}  & -     &  -      &  31.7\% & 41.5\% & 26.8\%   & - & - & - & - & - & - & - & - & 41\\  \hline
    \textbf{Openwrt}  & -     &  -      &  - & - & -   & - & - & - & - & - & 44.4\% & 55.6\% & - & 3837\\  \hline
    \textbf{Tenda-zh}  & -  &  - &  1.4\% & 10.2\%   & 15.6\% & 16.3\% & 16.3\% & 13.6\% & 9.5\% & 10.2\% & 6.8\% & - & - & 147\\  \hline
    \textbf{Trendnet}  & 0.2\%  &  - &  0.7\% & 0.2\%   & - & - & 69.2\% & 9.5\% & 3.7\% & 3.7\% & 14.9\% & 1.5\% & - & 409\\  \hline
    \textbf{Tenda-en}  & 0.6\%     &  8.5\% &  9.7\% & 10.3\%   & 13.9\% & 5.5\% & 13.3\% & 4.8\% & 7.9\% & 9.7\% & 7.3\% & 8.5\% & - & 165\\  \hline
    \textbf{Tplink-zh}  & 5.5\%  &  3.7\% & 4.5\%  & 10.0\%   & 5.9\% & 5.9\% & 2.4\% & 1.6\% & 1.6\% & 17.4\% & 31.6\% & 2.3\% & 7.4\% & 992\\  \hline
    \textbf{tomato}  & -  &  - &  - & -   & 97.5\% & 1.6\% & 0.9\% & - & - & - & - & - & - & 321\\  \hline
    \textbf{Ublox}  & -  &  - &  - & -   & - & - & 3.2\% & 3.2\% & - & 9.7\% & 32.3\% & 32.3\% & 19.4\% & 15\\  \hline
    \textbf{ubiquiti}  & -  &  - &  - & -   & - & - & - & 31.5\% & 27.4\% & 27.4\% & 13.7\% & - & - & 73\\  \hline
    \textbf{Zyxel}  & -  &  - &  - & -   & - & - & - & 13.3\% & 6.7\% & 20.0\% & 53.3\% & 6.7\% & - & 31\\  \hline
    \textbf{AVM}        &  -   & -    & -    &   -   &   -   & - & - & - & - & - & - & - & 100\% & 107 \\  \hline
    \textbf{Belkin}     &  -    & -         & -         &   -   &   -   & - & - & - & - & - & - & - & 100\% & 165 \\  \hline
    \textbf{Camius}     & -         &  -        &    -      & - &   -   & - & - & - & - & - & - & - & 100\% & 6\\  \hline
    \textbf{Haxorware}  & -     &  -        &    -      & -     &   -   & - & - & - & - & - & - & - & 100\% & 2\\  \hline
    \textbf{Mikrotik}     &  -    & -         & -         &   -   &   -   & - & - & - & - & - & - & - & 100\% & 49 \\  \hline
    \textbf{Netgear}     &  -    & -         & -         &   -   &   -   & - & - & - & - & - & - & - & 100\% & 3682 \\  \hline
    \textbf{Supermirco}     &  -    & -         & -         &   -   &   -   & - & - & - & - & - & - & - & 100\% & 192 \\  \hline
     \textbf{Tplink-en}  & -  &  - &  - & -   & - & - & - & - & - & - & - & - & 100\% & 1186\\  \hline

    \hline
  \end{tabular}
  \vspace{-1.5em}
\end{table*}



==> tables/kernel-hardens.tex <==
\begin{table*}[ht]
  \centering
  \caption{Hardening Measures in Linux Kernel}
  \label{tab:kmeasure}
  \scriptsize
  \begin{tabular}{c c c c c}
    \hline\hline
     \textbf{Attack Vector} & \textbf{Mitigations} & \textbf{Build Configuration} & \textbf{Version} & Default\\ \hline
    Stack Overflow &  Stack Canary  &    CONFIG\_HAVE\_CC\_STACKPROTECTOR   &   v2.6.30  & \checkmark  \\  \hline
    Stack Overflow &  Stack Canary &  CONFIG\_HAVE\_CC\_STACKPROTECTOR\_STRONG   &   v3.14  &\checkmark  \\  \hline
    Stack Overflow &  Virtually Mapped Kernel   &   CONFIG\_HAVE\_ARCH\_VMAP\_STACK   &   x86:v4.9 aarch64:v4.14  & \ding{55}  \\  \hline
    Buffer Overflow &  Fortify Source   &   CONFIG\_FORTIFY\_SOURCE   &   v4.13  & \ding{55} \\  \hline
    % \textbf{stack overflow} &  linked-list hardening   &   CONFIG\_DEBUG\_LIST   &   v4.10    \\  \hline
    % Heap Overflow &  Heap Obfuscation   &   CONFIG\_SLUB\_HARDENED   &   v4.14    \\  \hline
    Heap Overflow &  Non-exec Memory   &   CONFIG\_STRICT\_KERNEL\_RWX   &   v4.11  & \checkmark  \\  \hline
    Heap Overflow &  Harden Usercopy   &   CONFIG\_HARDENED\_USERCOPY   &   v4.8  & \ding{55}  \\  \hline
    Heap Overflow &  Freelist Randomization   &   CONFIG\_SLAB\_FREELIST\_RANDOM   &  v4.7   & \ding{55} \\  \hline
    %SLUB:v4.7  SLUB:v4.8
    Integer Overflow &  PAX\_REFCOUNT   &   Merged in Source   &   v4.11  & \checkmark \\  \hline
    Execution/Data Access &  SMEP  &   Merged in Source   &   x86:v3.0  & \checkmark \\  \hline
    Execution/Data Access &  SMAP  &   Merged in Source   &   x86:v3.7  & \checkmark \\  \hline
    Execution/Data Access &  PXN   &   Merged in Source   &   armv7:v3.19 arm64:v3.7  & \checkmark\\  \hline
    % Overflow &  W\&X detection   &   CONFIG\_DEBUG\_WX   &   x86:v4.4  arm64:v4.10  \\  \hline
    Kernel Exposure &  KASLR   &  CONFIG\_RANDOMIZE\_BASE   &   x86:v3.14 arm64:v4.6  mips:v4.7 & \ding{55} \\  \hline
    \hline
  \end{tabular}
  \vspace{-1.5em}
\end{table*}

==> tables/kernel-mitigation-vendor.tex <==
\setlength\tabcolsep{8pt}
\begin{table*}[!t]
  \centering
  \caption{Breakdown results of adoption of kernel-level mitigations.}
  \label{tab:kernel-mitigation-vendor}
  \footnotesize
  \begin{tabular}{ l | c| c| c| c| c| c| c| c}
    \toprule
    \textbf{Vendor} & \textbf{Total} & \textbf{Canary} & \textbf{PXN} &\textbf{KASLR} & \textbf{FreeList} & \textbf{Usercopy} & \textbf{Fortify} & \textbf{Kernel RWX}\\\toprule
    CenturyLink & 1 & 0 & -  & -   & - & - & - & -  \\ \hline
    Digi & 1 & - & - & -   & - & - & - & -  \\ \hline
    360 & 2 & 0 & -  & 0   & 0 & 0 & - & -  \\ \hline
    Buffalo & 2 & 2 & -  &  0  & 0 & 0 & - &  - \\ \hline
    Phicomm & 3 & 0 & -  & 0   & 0 & 0 & - & -  \\ \hline
    Zyxel & 3 & 0 &  0 & 0   & 0 & 0 & 0 &  0 \\ \hline
    Camius & 6 & 1 &  1 &  0  & 0 & 0 & 0 & 0  \\ \hline
    Supermicro & 6 & 0 & 0  &  -  & 0 & 0 & - &  - \\ \hline
    Openwrt & 9 & 9 & 9  &  0  & 0 & 3 & 4 & 5  \\ \hline
    Polycom & 16 & - & -  & -   & - & - & - & -   \\\hline
    TomatoShibby & 23 & 0 & 0  & 0   & 0 & - & - &  - \\ \hline
    Mercury & 27 & 0 & -  &  -  & - & - & - & -  \\ \hline
    Belkin & 33 & 0 & -  &  0  & 0 & 0 & - & -  \\ \hline
    TRENDnet & 71 & 0 & 0  &  0  & 0 & 0 & 0 & 0  \\ \hline
    Linksys & 75 & 8 &  3 &  0  & 0 & 0 & 0 & 0  \\ \hline
    Netcore & 85 & 0 & 1  &  0  & 0 & 0 & 0 & 0  \\ \hline
    Dlink & 91 & 0 &  0 &  0  & 0 & 0 & 0 & 0  \\ \hline
    Tenda & 118 & 0 & 0  &  0  & 0 & 0 & 0 & 0  \\ \hline
    Hikvision & 189 & 13 & 16  &  0  & 0 & 0 & 0 & 0  \\ \hline
    Tp-Link-zh & 325 & 7 & 2  & 0   & 0 & 0 & 0 & 1  \\ \hline
    ASUS & 319 & 0 & -  &  0  & 0 & 0 & - & -  \\ \hline
    Ubiquiti & 436 & 20 &  0 &  0  & 0 & 0 & - & 1  \\ \hline
    Tp-Link-en & 544 & 8 & 3  &  0  & 0 & 0 & 0 & 0  \\ \hline
    
    Netgear & 957 & 91 & 6  &  0  & 0 & 0 & 0 & 2  \\
    \bottomrule
    
  \end{tabular}
  \vspace{-1.5em}
\end{table*}
\setlength\tabcolsep{6pt}

==> tables/mitigation-product-change.tex <==
\setlength\tabcolsep{6pt}
\begin{table}[!t]
  \centering
  \caption{Mitigation Change of Multi-Version Products}
  \label{tab:mitigation-product-change}
  \scriptsize
  \begin{tabular}{ c| c| c| c| c| c}
    \hline\hline
    \textbf{\# Product} & \textbf{Canary} & \textbf{RELRO} &\textbf{NX} & \textbf{Fortify} & \textbf{PIE} \\\hline
    699 & +83/-121 & +50/143 & +99/-37 & +51/-85 & +203/-297 \\ \hline
  \end{tabular}
  \vspace{-1.5em}
\end{table}
\setlength\tabcolsep{6pt}

==> tables/nx-pie.tex <==
\begin{table}[t]
  \centering
  \caption{Analysis of Non-exec Stack and PIE}
  \label{tab:nx-pie}
  \scriptsize
  \begin{tabular}{ c| c| c| c}
    \hline\hline
    \textbf{Vendor} & \textbf{ELF (k)} & \textbf{NX} & \textbf{PIE}\\\hline
    Haxorware & 0.2 & 0 & 14.9   \\ \hline
    Actionec & 0.4 & 47.2 & 13.4     \\ \hline
    Cerowrt & 0.4 & 0 & 9.8   \\ \hline
    360 & 0.5 & 0 & 8.9   \\ \hline
    Buffalo & 0.5 & 45.8 & 6.0\\ \hline
    Camius & 0.5 & 92.1 & 11.9    \\ \hline 
    AT\&T  & 0.6 & 0 & 6.3  \\ \hline
    CenturyLink & 0.8 & 0 & 0.6  \\ \hline
    Zyxel & 0.8 & 97.3 & 11.6  \\ \hline
    GOCloud & 0.9 & 98.2 & 14.9  \\ \hline
    TENVIS & 0.9 & 0 & 34.0  \\ \hline
    Supermicro & 1.3 & 97.8 & 18.5  \\ \hline
    Digi & 1.3 & 3.5 & 18.5  \\ \hline
    Mercury & 1.5 & 0 & 31.5  \\ \hline
    Phicomm & 1.9 & 21.2 & 47.2  \\ \hline
    MikroTik & 4.3 & 81.0 & 5.8  \\ \hline
    AVM & 5 & 95.6 & 90.8  \\ \hline
    Belkin & 7.9 & 7.4 & 11.0  \\ \hline
    NETCore & 10.2 & 0.06 & 16.4  \\ \hline
    TRENDnet & 15.3 & 10.1 & 13.6  \\ \hline
    Dlink & 15.9 & 30.4 & 9.1 \\ \hline
    Linksys & 17.1 & 60.4 & 9.0  \\ \hline
    RouterTech & 25.8 & 0 & 15.0  \\ \hline
    Moxa & 32.0 & 75.7 & 31.8  \\ \hline
    Tenda & 33.6 & 30.5 & 11.7  \\ \hline
    Tp-Link-zh & 65.7 & 38.7 & 18.3  \\ \hline
    Tp-Link-en & 76.3 & 36.6 & 21.5  \\ \hline
    TomatoShibby & 127.8 & 23.2 & 8.4  \\ \hline
    NETGEAR & 173.9 & 55.9 & 11.4  \\ \hline
    OpenWrt & 191.2 & 99.9 & 0  \\ \hline
    Ubiquiti & 204.7 & 15.6 & 9.5  \\ \hline
    ASUS & 273.2 & 46.8 & 8.3  \\ \hline
    QNAP & 296 & 99.2 & 7.7  \\ \hline
    Synology & 1375.4 & 99.5 & 13.5  \\ \hline
    \hline
  \end{tabular}
  \vspace{-1.5em}
\end{table}

==> tables/product-eval.tex <==
\begin{table}[t]
  \centering
  \caption{Binary Mitigation Changes cross Product Version}
  \label{tab:product-eval}
  \scriptsize
  \begin{tabular}{ c| c| c| c}
    \hline\hline
    & \textbf{Overlap ELF} & \textbf{Positive Change} & \textbf{Negative Change}\\ \hline
    \textbf{Canary} & 3089 & 361 & 7\\ \hline
    \textbf{Fortify} & &  & \\ \hline
    \textbf{RELRO} & &  & \\ \hline
    \textbf{NX} & &  & \\ \hline
  \end{tabular}
  \vspace{-1.5em}
\end{table}

==> tables/related-work.tex <==

\begin{table*}[t!]
  \centering
  \caption{Related Work in Category}
  \label{tab:related}
  \scriptsize
  \begin{tabular}{c c c c c}
    \hline\hline
    \textbf{Name} & \textbf{Static Analysis} & \textbf{Dynamic Analysis}  &   \textbf{Defense Assessment} & \textbf{Firmware \#} \\\hline
    \textbf{BINWARM}\cite{shirani2018binarm}   & \checkmark   &      &      & 5756      \\  \hline
    \textbf{GENIUS}\cite{feng2016scalable}   & \checkmark   &      &        & 8128    \\  \hline
    \textbf{FirmUp}\cite{david2018firmup}   & \checkmark   &      &        & 2000    \\  \hline
    \textbf{Firmware Analysis}\cite{costin2014large}   & \checkmark   &      &      & 32356      \\  \hline
    
    \textbf{discoverRE}\cite{eschweiler2016discovre}   & \checkmark   &      &      &   2   \\  \hline
    \textbf{Automated Dynamic Analysis}\cite{chen2016towards}     &    &   \checkmark    &    & 8617   \\  \hline
    \textbf{MULTI-MH}\cite{pewny2015cross}   &    &  \checkmark    &      &     2  \\  \hline
    \textbf{FirmFuzz}\cite{srivastava2019firmfuzz}     &    &   \checkmark    &       \\  \hline
    \textbf{SoK: HomeBased IoT Deployment}\cite{alrawi2019sok}   &    &   \checkmark    &            \\  \hline
    \textbf{Analysis on Embedded Web Interface}\cite{10.1145/2897845.2897900}  &    &   \checkmark    &            \\  \hline
    \textbf{28 Routers}\cite{buildsafety}   &    &       & \checkmark   & 28    \\  \hline
    \textbf{uArmor}\cite{abbasi2019challenges}   &    &       & \checkmark       \\  \hline
    \hline
  \end{tabular}
\end{table*}


==> tables/stc-files-eval.tex <==
\begin{table}[t]
  \centering
  \caption{Stack Canary and Fortify Source Evaluation of Statically Linked Binaries \studentfix{all fortify found from synology}}
  \label{tab:stc-result}
  \scriptsize
  \begin{tabular}{ c| c| c| c}
    \hline\hline
    & \textbf{Num} & \textbf{Canary \#} & \textbf{Fortify \#}\\ \hline
    \textbf{STC Stripped Binaries} & 8370 & 697 & 651\\ \hline
  \end{tabular}
  \vspace{-1.5em}
\end{table}

==> tables/tools_comparison.tex <==
\begin{table}[t]
  \centering
  \caption{Analysis of Binary Hardening Measure}
  \label{tab:tools-comparison}
  \scriptsize
  \begin{tabular}{ c| c| c| c| c| c| c}
    \hline\hline
    & \textbf{PIE} & \textbf{NX} & \textbf{Canary} & \textbf{Fortify} & \textbf{RELRO}  & \textbf{ELF}\\ \hline
    \textbf{Self} & 60.1 & 43.8 & 30.1 & 22.8 & 18.6 & \multirow{3}{*}{2920540}\\ \cline{1-6}
    \textbf{Pwntool} & 60.1 & 43.8 &  &  &  & \\ \cline{1-6}
    \textbf{CheckSec} & - & 43.8 &  &  &  & \\ \hline
  \end{tabular}
  \vspace{-1.5em}
\end{table}

==> tables/user-space.tex <==
\begin{table*}[ht]
  \centering
  \caption{Attack mitigations in Linux-based binary programs.}
  \label{tab:user-space}
  \small
  \begin{tabular}{ c c l c}
    \toprule
    \textbf{Attack Vector} & \textbf{Mitigation} & \textbf{First Release} & \textbf{Default}$^{1}$\\
    \toprule
    Stack Overflow &  Stack Canaries  &    2005 (GCC)  &   \ding{51} \\\hline
    GOT Hijacking &  Relocation Read-Only  & 2004 (GCC) &   \ding{51} \\\hline
    Code Injection &  Non-Executable Stack  &    2003 (GCC) &   \ding{51} \\\hline
    Buffer Overflow &  Fortify Source  &    2004 (GLIBC)  &   \ding{51} \\\hline
    Control-flow Hijacking & Position-Independent (or ASLR-Capable) Code &    2003 (GCC)  & \ding{51} \\ \hline
    Heap Overflow & Heap Checks by libc & 2004 (GLIBC) & \ding{51} \\
    \bottomrule
    
    \multicolumn{4}{ l }{$^{1}$~In Debian 10
    ``buster,'' released in July 2019, GCC v8.3.0}
  \end{tabular}
\end{table*}

==> tables/vulnerability-mitigation.tex <==
\setlength\tabcolsep{4.6pt}
\begin{table}[t!]
  \centering
  \caption{\textcolor{blue}{Mitigation adoption rates (\%) on vulnerable binaries.}}
  \label{tab:vulnerable-mitigation}
  \begin{tabular}{l c c c c c}
    \toprule
    \textbf{} & \textbf{Canary} & \textbf{RELRO} & \textbf{NX} & \textbf{Fortify} & \textbf{PIE}\\ \toprule
    \textbf{Realtek}      & 3.5    & 1.6    & 24.4    & 0.1    & 2.5\\  \bottomrule
  \end{tabular}
\end{table}
\setlength\tabcolsep{6pt}
